ReFACT: Updating Text-to-Image Models by Editing the Text Encoder

Our world is marked by unprecedented technological, global, and socio-political transformations, posing a significant challenge to text-to-image generative models. These models encode factual associations within their parameters that can quickly become outdated, diminishing their utility for end-users. To that end, we introduce ReFACT, a novel approach for editing factual associations in text-to-image models without relaying on explicit input from end-users or costly re-training. ReFACT updates the weights of a specific layer in the text encoder, modifying only a tiny portion of the model's parameters and leaving the rest of the model unaffected. We empirically evaluate ReFACT on an existing benchmark, alongside a newly curated dataset. Compared to other methods, ReFACT achieves superior performance in both generalization to related concepts and preservation of unrelated concepts. Furthermore, ReFACT maintains image generation quality, making it a practical tool for updating and correcting factual information in text-to-image models.

==> tables/line_search.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\caption{Hyper-parameter Tuning on RoAD.}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccc|llll}
\textbf{} & \textbf{Layer} & \textbf{lr} & \textbf{thr} & \textbf{stp} & \multicolumn{1}{c}{\textbf{Efficacy} ($\uparrow$)} & \multicolumn{1}{c}{\textbf{Generalization} ($\uparrow$)} & \multicolumn{1}{c}{\textbf{Specificity} ($\uparrow$)} & \multicolumn{1}{c}{\textbf{Mean} ($\uparrow$)} \\ \hline
\multirow{11}{*}{} & 0 & 0.5 & 0.99 & 50 & 100\% & 85.84\% & 93.52\% & 92.94\% \\
 & 1 & 0.5 & 0.99 & 50 & 100\% & 88.96\% & 92\% & 93.54\% \\
 & 2 & 0.5 & 0.99 & 50 & 100\% & 83.84\% & 94.32\% & 92.47\% \\
 & 3 & 0.5 & 0.99 & 50 & 100\% & 88.24\% & 93.12\% & 93.66\% \\
 & 4 & 0.5 & 0.99 & 50 & 100\% & 83.76\% & 94.16\% & 92.39\% \\
 & 5 & 0.5 & 0.99 & 50 & 100\% & 83.2\% & 92.72\% & 91.71\% \\
 & 6 & 0.5 & 0.99 & 50 & 100\% & 91.36\% & 90\% & 93.68\% \\
 & \textbf{7} & \textbf{0.5} & \textbf{0.99} & \textbf{50} & \textbf{100\%} & \textbf{96.96\%} & \textbf{94\%} & \textbf{96.96\%} \\
 & 8 & 0.5 & 0.99 & 50 & 100\% & 94.08\% & 90.56\% & 94.8\% \\
 & 9 & 0.5 & 0.99 & 50 & 100\% & 91.92\% & 95.2\% & 95.65\% \\
 & 10 & 0.5 & 0.99 & 50 & 99.6\% & 90.64\% & 96.16\% & 95.39\% \\ \hline
 & 7 & 0.05 & 0.99 & 50 & 99.6\% & 95.04\% & 95.04\% & 96.54\% \\ \hline
\multirow{2}{*}{} & 7 & 0.05 & 0.9 & 50 & 99.6\% & 94.16\% & 94.56\% & 96.08\% \\
 & 7 & 0.05 & 0.95 & 50 & 100\% & 91.76\% & 95.76\% & 95.78\% \\ \hline
\multirow{2}{*}{} & 7 & 0.05 & 0.99 & 15 &  &  &  & \multicolumn{1}{c}{} \\
 & 7 & 0.05 & 0.99 & 100 & 99.2\% & 92\% & 96.48\% & \textbf{95.85\%}
\end{tabular}%
}
\end{table}
